Posterior contraction and uncertainty quantification for the multivariate spike-and-slab LASSO

We study the asymptotic properties of Deshpande et al.\ (2019)'s multivariate spike-and-slab LASSO (mSSL) procedure for simultaneous variable and covariance selection in the sparse multivariate linear regression problem. In that problem, $q$ correlated responses are regressed onto $p$ covariates and the mSSL works by placing separate spike-and-slab priors on the entries in the matrix of marginal covariate effects and off-diagonal elements in the upper triangle of the residual precision matrix. Under mild assumptions about these matrices, we establish the posterior contraction rate for the mSSL posterior in the asymptotic regime where both $p$ and $q$ diverge with $n.$ By ``de-biasing'' the corresponding MAP estimates, we obtain confidence intervals for each covariate effect and residual partial correlation. In extensive simulation studies, these intervals displayed close-to-nominal frequentist coverage in finite sample settings but tended to be substantially longer than those obtained using a version of the Bayesian bootstrap that randomly re-weights the prior. We further show that the de-biased intervals for individual covariate effects are asymptotically valid.

==> proofs.tex <==
% Proof of 
Recall the main assumptions needed for our theoretical analysis of the mSSL:
\begin{description}
\item[A1]{$\Omega_{0}$ has bounded operator norm and eigenvalues; that is, 
$$
\Omega_{0} \in \mathcal{H}_{0} = \{\Omega: \text{all of $\Omega$'s eigenvalues lie in $[b_{1}^{-1}, b_{2}^{-1}]$}\},
$$ where $b_{1}, b_{2}$ are fixed constants not depending on $n.$}
\item[A2]{$B_{0}$ has bounded entries; that is, $B_{0} \in \mathcal{B}_{0} = \{B: \lVert B \rVert_{\infty} < a_{1}\}$ where $a_{1} > 0$ is a fixed constant not depending on $n.$}
\item[A3]{Dimensionality; $\log(n) \lesssim \log(q), \log(n) \lesssim \log(p)$ and 
$$
\max\{q,s_0^\Omega,s_0^B\}\log(\max\{p,q\})/n\to 0.
$$}
\item[A4]{Prior tuning for $B$; there are constants $a' > 0$ and $b' > 1/2$ that do not depend on $n$ such that (i)$(1-\theta)/\theta\sim (pq)^{2+a'}$; (ii) $\lambda_0\sim \max\{n,pq\}^{2+b'}$; and (iii) $\lambda_1\asymp  1/n.$}
\item[A5]{Prior tuning for $\Omega;$ there are constants $a,b > 0$ not depending on $n$ such that (i) $(1-\eta)/\eta\sim Q^{2+a}$; (ii) $\xi_0\sim \max\{Q,n\}^{4+b}$; and (iii) $\xi_1\asymp 1/\max\{Q,n\}$.}
\end{description}

Under these assumptions, our prior densities are

\begin{align}
    \begin{split}
        p(\Omega \vert \eta) & \propto \prod_{k>k'}\left[\frac{(1-\eta) \xi_0}{2}\exp\left(-\xi_0|\omega_{k,k'}|\right)+\frac{\eta\xi_1}{2}\exp\left(\xi_1|\omega_{k,k'}|\right)\right] \\
        ~&~~~\times \prod_{k}\xi_1\exp\left[-\xi_1\omega_{k,k}\right] \times \mathbbm{1}(\Omega\succ \tau I) 
        \end{split}
        \\
        p(B\vert\theta) & =\prod_{jk}\left[\frac{(1-\theta) \lambda_0}{2}\exp\left(-\lambda_0|\beta_{j,k}|\right)+\frac{\theta\lambda_1}{2}\exp\left(\lambda_1|\beta_{j,k}|\right)\right]
\end{align}

%\skd{In A1, we use $b_{1}^{-1}$ as the lower bound on eigenvalues. But in proofs we use $\tau.$ I propose we switch $\tau$ to $b_{1}^{-1}.$}
%\yunyi{They are different things, $b_1$ are for the true $\Omega$ while $\tau$ is a truncation on the prior.}


Before proceed, we restate Lemma S3 from \citet{shen2022cgSSL} that allows us to bound probabilities with respect to the prior on $\Omega$ by considering an untruncated version of the prior.

\begin{myLemma}
    Let $\tilde{\Pi}$ be the untruncated version of the prior on $\Omega.$
    Then for all events $A,$ for large enough $n$ there is a number $R$ that does not depend on $n$ such that
        \begin{equation}
            \label{eqn:graphical_prior_bound}
            \tilde{\Pi}(\Omega\succ \tau I|A)\tilde{\Pi}(A)\le \Pi_\Omega(A\cap \{\Omega\succ \tau I\})\le \exp(2 \xi_1 Q-\log(R))\tilde{\Pi}(A)
        \end{equation}
        where $Q=q(q-1)/2$ is the total number of free off-diagonal entries in $\Omega.$
\end{myLemma}

\subsection{Proof of Lemma 1}

The KL divergence between a multivariate regression model with parameters $(B_{0},\Omega_{0})$ and one with parameters $(B,\Omega)$ is
\begin{equation}
\label{eqn:KL_formula}
K(f_{0}, f) = \frac{n}{2}\left(\log\left(\frac{|\Omega_0|}{|\Omega|}\right)-q+\tr(\Omega_0^{-1}\Omega)+\frac{1}{n}\tr\left\{ (B_0-B)^{\top}X^{\top}X(B_0-B)\Omega \right\}\right).
\end{equation}
The KL variance between the same models is 
\begin{equation}
\label{eqn:KLv_formula}
V(f_{0}, f) = \frac{n}{2}\left(\tr((\Omega_0^{-1}\Omega)^2)-2\tr (\Omega_0^{-1}\Omega) + q \right)+\frac{1}{n}\tr\left((B-B_0)^{\top}X^{\top}X(B-B_0)\Omega\Omega_0^{-1}\Omega\right).
\end{equation}

%We first obtain an upper bound of the average KL divergence and variance so that the mass of such event can serve as a lower bound. 
%\skd{This sentence is very hard to parse!!}
Observe that both KL divergence and KL variance has term that only depends on $\Omega$ and term depends on both $B$ and $\Omega$. We separate the two type of terms and bound them separately.

To simplify the notation, we denote $(B-B_0)=\Delta_B$ and $\Omega-\Omega_0=\Delta_\Omega$. 
Consider the events $\mathcal{A}_{1}$ and $\mathcal{A}_{2}$ defined as
\begin{equation}
    \label{eqn:mssl_A1_due_to_Omega}
    \mathcal{A}_1=\left\{ \Omega: \tr((\Omega_0^{-1}\Omega)^2)-2\tr (\Omega_0^{-1}\Omega) + q\le \epsilon_n^2, \log\left(\frac{|\Omega_0|}{|\Omega|}\right)-q+\tr(\Omega_0^{-1}\Omega)\le \epsilon_n^2 \right\}
\end{equation}
and
\begin{equation}
    \label{eqn:mssl_A2_condition_on_A1}
    \begin{aligned}
        \mathcal{A}_2=\{ (\Omega, B): &\tr\left\{ (B_0-B)^{\top}X^{\top}X(B_0-B)\Omega \right\}\le n\epsilon^2,\\ &\tr\left((B-B_0)^{\top}X^{\top}X(B-B_0)\Omega\Omega_0^{-1}\Omega\right)  \le n\epsilon_n^2/2  \}\\
    \end{aligned}
\end{equation}

By construction the event $\mathcal{A}_1$ involves only $\Delta_\Omega$ and the event $\mathcal{A}_2$ involves both $\Delta_\Omega$ and $\Delta_B.$  
Further, the event $(\mathcal{A}_1\cap \{\Omega\succ \tau I\})\cap \mathcal{A}_2$ is a subset of the event  $\{ K/n\le \epsilon_n^2, V/n\le\epsilon_n^2 \}$. To show the lemma, it suffices to lower bound $\log\Pi(\mathcal{A}_1)+\log\Pi(\mathcal{A}_1|\mathcal{A}_2)$ with the stated lower bound. We separately bound the prior probabilities $\Pi(\mathcal{A}_1)$ and $\Pi(\mathcal{A}_1|\mathcal{A}_2)$.


We start with lower bound the prior mass put on $\mathcal{A}_1$. We consider a smaller set, the vectorized L1 ball $\mathcal{A}_1^\star$:
\begin{align*}
    \mathcal{A}_1^\star=\{2\sum_{k>k'} |\omega_{0,k,k'}-\omega_{k,k'}|+\sum_k |\omega_{0,k,k}-\omega_{k,k}|\le \frac{\epsilon_n}{b_2}\}%\subset\{||\Omega_0-\Omega||_F\le \frac{\epsilon_n}{c_1\sqrt{p}}\}\subset \mathcal{A}_1
\end{align*}
where $b_{2} > 0$ is the constant in the assumption of $\Omega_0$'s spectra.

Since the Frobenius norm is bounded by the vectorized L1 norm, we conclude that 
$$
A_{1}^{\star} \subset \left\{ \lVert \Omega_{0} - \Omega \rVert_{F} \leq \frac{\epsilon_{n}}{b_{2}}\right\}.
$$
We now show that $\left\{ \lVert \Omega_{0} - \Omega \rVert_{F} \leq \frac{\epsilon_{n}}{b_{2}} \right\}\subset \mathcal{A}_1$.

Per \citet{Ning2020}'s Lemma 5.1, using our assumption that $\Omega_0$'s eigenvalue was bounded by $1/b_2\le \lambda_{\min}\le \lambda_{\max}\le 1/b_1$, we have, for sufficiently large $n,$ $\{||\Omega_0-\Omega||_F\le \epsilon_n/b_2\}\subset \mathcal{A}_1.$
Because the
absolute value of the eigenvalues of $\Delta_\Omega$ are bounded by $\epsilon_n/b_2$, for sufficiently large $n$ (i.e. small enough $\epsilon_n$) -- the spectra of $\Omega=\Omega_0+\Delta_\Omega$ is bounded by $\lambda_{\min}-\epsilon_n/b_2$ and $\lambda_{\max}+\epsilon_n/b_2$ and can be further bounded by $\lambda_{\min}/2$ and $2\lambda_{\max}$ when $n$ is large. Thus we can conclude $\tilde{\Pi}(\Omega\succ \tau I|\mathcal{A}_1^\star)=1$ when $n$ is large enough. 

Consequently, we can bound the prior mass $\Pi(\mathcal{A}_1)$ by bounding the prior mass on $\Pi(\mathcal{A}_1^\star)$. Instead of calculating the probability directly, we can lower bound it by observing that
\begin{align*}
    &2\sum_{k>k'} |\omega_{0,k,k'}-\omega_{k,k'}|+\sum_k |\omega_{0,k,k}-\omega_{k,k}|\\
    =&2\sum_{(k,k')\in S_0^\Omega} |\omega_{0,k,k'}-\omega_{k,k'}| + 2\sum_{(k,k')\in (S_0^\Omega)^c} |\omega_{k,k'}|+\sum_{k} |\omega_{0,k,k}-\omega_{k,k}|
\end{align*}

Consider the following events:
\begin{align*}
    \mathcal{B}_1&=\{ \sum_{(k,k')\in S_0^\Omega} |\omega_{0,k,k'}-\omega_{k,k'}|\le \frac{\epsilon_n}{6b_2}  \}\\
    \mathcal{B}_2&=\{\sum_{(k,k')\in (S_0^\Omega)^c} |\omega_{k,k'}|\le \frac{\epsilon_n}{6b_2}\}\\
    \mathcal{B}_3&=\{ \sum_{k} |\omega_{0,k,k}-\omega_{k,k}| \le  \frac{\epsilon_n}{3b_2}\} \}
\end{align*}
Let $\mathcal{B}=\bigcap_{i=1}^3\mathcal{B}_i\subset \mathcal{A}_1^*\subset \mathcal{A}_1$. Since the prior mass on $\mathcal{B}$ using the lower bound in ~\eqref{eqn:graphical_prior_bound}, we can focus on estimating $\tilde{\Pi}(\mathcal{B})$. Using the fact that $\tilde{\Pi}$ is separable we have
\begin{align*}
    \Pi(\mathcal{A}_1\cap \{\Omega\succ \tau I\})\ge\Pi(\mathcal{A}_1^*\cap \{\Omega\succ \tau I\})\ge \tilde{\Pi}(\mathcal{A}_1^*)\ge \tilde{\Pi}(\mathcal{B})=\prod_{i=1}^3\tilde{\Pi}(\mathcal{B}_i).
\end{align*}

We bound the prior mass on $\mathcal{B}_1$ using pure slab part of the prior, the same technique used in \citet{Bai2020_groupSSL} (specifically Equation D.18). We have
\begin{align*}
\tilde{\Pi}(\mathcal{B}_1)&=\int_{\mathcal{B}_1}\prod_{(k,k')\in S_0^\Omega}   \pi(\omega_{k,k'}|\eta)d\mu\\
&\ge \prod_{(k,k')\in S_0^\Omega}  \int_{|\omega_{0,k,k'}-\omega_{k,k'}|\le \frac{\epsilon_n}{6s_0^\Omega b_2}} \pi(\omega_{k,k'}|\eta) d\omega_{k,k'}\\
&\ge \eta^{s_0^\Omega} \prod_{(k,k')\in S_0^\Omega}  \int_{|\omega_{0,k,k'}-\omega_{k,k'}|\le \frac{\epsilon_n}{6s_0^\Omega b_2}} \frac{\xi_1}{2} \exp(-\xi_1|\omega_{k,k'}|) d\omega_{k,k'}\\
&\ge \eta^{s_0^\Omega} \exp(-\xi_1\sum_{(k,k')\in S_0^\Omega}|\omega_{0,k,k'}|)\prod_{(k,k')\in S_0^\Omega}  \int_{|\omega_{0,k,k'}-\omega_{k,k'}|\le \frac{\epsilon_n}{6s_0^\Omega b_2}} \frac{\xi_1}{2} \exp(-\xi_1|\omega_{0,k,k'}-\omega_{k,k'}|) d\omega_{k,k'}\\
&=\eta^{s_0^\Omega}\exp(-\xi_1||\Omega_{0,S_0^\Omega}||_1) \prod_{(k,k')\in S_0^\Omega} \int_{|\Delta| \le \frac{\epsilon_n}{6s^\Omega_0b_2}}\frac{\xi_1}{2} \exp(-\xi_1|\Delta|)d\Delta\\
&\ge \eta^{s_0^\Omega}\exp(-\xi_1||\Omega_{0,S_0^\Omega}||_1)\left[e^{-\frac{\xi_1\epsilon_n}{6b_2s^\Omega_0}}\left(\frac{\xi_1\epsilon_n}{6s^\Omega_0b_2}\right)\right]^{s^\Omega_0}.
\end{align*}

The first inequality holds because the fact that $|\omega_{0,k,k'}-\omega_{k,k'}|\le \epsilon_n/(6s_0^\Omega b_2)$ implies the sum less than $\epsilon_n/(6 b_2)$. The last inequality is a special case of Equation D.18 of \citet{Bai2020_groupSSL}

For $\mathcal{B}_2$ we derive the lower bound using the spike component of the prior. Let $Q=q(q-1)/2$ denote the number of off-diagonal entries of matrix $\Omega$. 
\begin{align*}
\tilde{\Pi}(\mathcal{B}_2)&=\int_{\mathcal{B}_2}\prod_{(k,k')\in (S_0^\Omega)^c}   \pi(\omega_{k,k'}|\eta)d\mu\\
&\ge \prod_{(k,k')\in (S_0^\Omega)^c} \int_{|\omega_{k,k'}|\le \frac{\epsilon_n}{6(Q-s_0^\Omega)b_2}} \pi(\omega_{k,k'}|\eta)d\mu\\
&\ge (1-\eta)^{Q-s_0^\Omega} \prod_{(k,k')\in (S_0^\Omega)^c} \int_{|\omega_{k,k'}|\le \frac{\epsilon_n}{6(Q-s_0^\Omega)b_2}} \frac{\xi_0}{2} \exp(-\xi_0|\omega_{k,k'}|)d\omega_{k,k'} \\
&\ge(1-\eta)^{Q-s_0^\Omega}\prod_{(k,k')\in (S_0^\Omega)^c}\left[1-\frac{6(Q-s_0^\Omega)b_2}{\epsilon_n}\mathbb{E}_{\pi}|\omega_{k,k'}|\right]\\
&=(1-\eta)^{Q-s_0^\Omega}\left[1-\frac{6(Q-s_0^\Omega)b_2}{\epsilon_n\xi_0}\right]^{Q-s_0^\Omega}\\
&\gtrsim (1-\eta)^{Q-s_0^\Omega} \left[1-\frac{1}{Q-s_0^\Omega}\right]^{Q-s_0^\Omega}\\
&\asymp (1-\eta)^{Q-s_0^\Omega}.
\end{align*}

To derive the last two lines we used the similar argument used by \citet{Bai2020_groupSSL}'s D.22 to establish that $1-\frac{6(Q-s_0^\Omega)b_2}{\epsilon_n\xi_0}\gtrsim 1-1/(Q-s_0^\Omega)$. 
That is, recall our assumption that $\xi_0\sim \max\{Q,n\}^{4+b}$; this assumption allows us to control the $Q$ term and $n$ term induced by $\epsilon_n$ appearing in the numerator in the fifth line.
Because $s_0^\Omega$ grows slower than $Q$, we have $Q-s_0^\Omega\to\infty$ thus we can lower bound the above function using some constant multiple of $(1-\eta)^{Q-s_0^\Omega}$.  
%Directly applying the same argument in \citet{shen2022cgSSL}, we conclude 

The event $\mathcal{B}_3$ depends only on the diagonal entries of $\Omega$. 
The prior mass can be directly bounded using results on exponential distributions. 
\begin{align*}
\tilde{\Pi}(\mathcal{B}_3)&=\int_{\mathcal{B}_3}\prod_{i=1}^q   \pi(\omega_{k,k})d\mu\\
&\ge \prod_{i=1}^q  \int_{|\omega_{0,k,k}-\omega_{k,k}|\le \frac{\epsilon_n}{3q b_2}} \pi(\omega_{k,k}) d\omega_{k,k}\\
&=\prod_{i=1}^q  \int_{\omega_{0,k,k}- \frac{\epsilon_n}{3 q b_2}}^{\omega_{0,k,k}+ \frac{\epsilon_n}{3 q b_2}} \xi_1 \exp(-\xi_1\omega_{k,k}) d\omega_{k,k}\\
&\ge \prod_{i=1}^q  \int_{\omega_{0,k,k}}^{\omega_{0,k,k}+ \frac{\epsilon_n}{3 q b_2}} \xi_1 \exp(-\xi_1\omega_{k,k}) d\omega_{k,k}\\
&=\exp(-\xi_1 \sum_{i=1}^q\omega_{0,k,k})\int_{0}^{ \frac{\epsilon_n}{3 q b_2}} \xi_1 \exp(-\xi_1\omega_{k,k}) d\omega_{k,k}\\
&\ge \exp(-\xi_1 \sum_{i=1}^q\omega_{0,k,k})\left[e^{-\frac{\xi_1\epsilon_n}{3b_2q}}\left(\frac{\xi_1\epsilon_n}{3qb_2}\right)\right]^{q}
\end{align*}


Now we can show the log prior mass on $\mathcal{B}$ can be lower bounded by some $\exp\{-C_1n\epsilon_n^2\}$, to this end, consider the negative log prior mass
\begin{align}
    \label{eq:B_event_for_Omega}
    \begin{split}
-&\log(\Pi(\mathcal{A}_1\cap \{\Omega\succ \tau I\}))\\
\le& \sum_{i=1}^3 -\log(\tilde{\Pi}(\mathcal{B}_i)) \\
\lesssim& -s_0^\Omega \log(\eta) + \xi_1||\Omega_{0,S_0^\Omega}||_1 + \frac{\xi_1 \epsilon_n}{6b_2}-s_0^\Omega \log\left(\frac{\xi_1\epsilon_n}{6s^\Omega_0b_2}\right)-
(Q-s_0^\Omega) \log(1-\eta)\\
&+\xi_1\sum_k \omega_{0,k,k}+\frac{\xi_1\epsilon_n}{3b_2}-q\log\left(\frac{\xi_1\epsilon_n}{3qb_2}  \right)\\
=&-\log\left( \eta^{s_0^\Omega} (1-\eta)^{Q-s_0^\Omega}  \right) + \xi_1||\Omega_{0,S_0^\Omega}||_1 + \frac{\xi_1 \epsilon_n}{6b_2}+\xi_1\sum_k \omega_{0,k,k}+\frac{\xi_1\epsilon_n}{3b_2}\\
&-s_0^\Omega \log\left(\frac{\xi_1\epsilon_n}{6s^\Omega_0b_2}\right)-q\log\left(\frac{\xi_1\epsilon_n}{3qb_2}  \right)\\
    \end{split}
\end{align}

The $\frac{\xi_1 \epsilon_n}{6b_2}$ and $\frac{\xi_1\epsilon_n}{3b_2}$ terms are of $O(\epsilon_n)\lesssim n\epsilon_n^2$. The 4th term is of order $q$ since the diagonal entries is controlled by the largest eigenvalue of $\Omega$ that was assumed to be bounded thus $\xi_1\sum_k \omega_{0,k,k}\lesssim n\epsilon_n^2$. Finally, 
\begin{align*}
\xi_1||\Omega_{0,S_0^\Omega}||_1\le \xi_1 s_0^\Omega \sup|\omega_{0,k,k'}|=O(s_0^\Omega)\lesssim n\epsilon_n^2
\end{align*}
because the entries of $\omega_{0,k,k'}$ is bounded. 

Without tuning $\eta$, the first term $-\log\left( \eta^{s_0^\Omega} (1-\eta)^{Q-s_0^\Omega}  \right)$ has order of $Q$.  
But since we assumed $\frac{1-\eta}{\eta}\sim Q^{2+a}$ for some $a>0$, we have $M_1 Q^{2+a} \le \frac{1-\eta}{\eta}\le M_2 Q^{2+a}$. That is, we have $1/(1+M_2 Q^{2+a})\le \eta \le 1/(1+M_1Q^{2+a})$, and a simple lower bound is:
\begin{align*}
\eta^{s_0^\Omega} (1-\eta)^{Q-s_0^\Omega}&\ge (1+M_2 Q^{2+a})^{-s_0^\Omega}(1-\eta)^{Q-s_0^\Omega}\\
&\ge (1+M_2 Q^{2+a})^{-s_0^\Omega}\left(1-\frac{1}{1+M_1Q^{2+a}}\right)^{Q-s_0^\Omega}\\
&\gtrsim (1+M_2 Q^{2+a})^{-s_0^\Omega}
\end{align*}

The last line is because $Q^{2+a}$ grows faster than $Q-s^\Omega_0$, thus $(1-\frac{1}{1+M_1Q^{2+a}})^{Q-s_0^\Omega}$ can be bounded below with some constant. 
Taking logarithms, we see 
\begin{align*}
-\log\left( \eta^{s_0^\Omega} (1-\eta)^{Q-s_0^\Omega}  \right) \lesssim s_0^\Omega \log(1+M_2 Q^{2+a})\lesssim s_0^\Omega \log(Q)\sim s_0^\Omega\log(q)\le \max(q,s_0^\Omega) \log(q).
\end{align*}

The last two terms in~\eqref{eq:B_event_for_Omega} can be treated in the same way, using our assumption that $\xi_1\asymp1/\max\{n,Q\}$:
\begin{align*}
-s_0^\Omega \log\left(\frac{\xi_1\epsilon_n}{6s^\Omega_0b_2}\right)&=s_0^\Omega \log\left(\frac{6s^\Omega_0b_2}{\xi_1\epsilon_n}\right)\\
&\lesssim s_0^\Omega \log\left(\frac{n^{1/2}\max\{n,Q\}s_0^\Omega }{\sqrt{\max\{s_0^\Omega,s_0^B,p,q\}\log(q)}}\right)\\
&\le s_0^\Omega \log\left(n^{1/2}\max\{n,Q\}s_0^\Omega \right)\\
&\lesssim s_0^\Omega\log(q^2)\\
&\lesssim n\epsilon_n^2
\end{align*}

The third line holds because $\max\{s_0^\Omega,s_0^B,p,q\}\log(q)\ge 1$ when $n$ is large.
The fourth line follows because(i)  $\log(n)\lesssim \log(q)$ by assumption and (ii) $s_0^\Omega <q^2$. 
The last line uses the definition of $\epsilon_n$.  

The last term in~\eqref{eq:B_event_for_Omega} can be bounded similar to the one before using our assumption about the slab penalty $\xi_1$:
\begin{align*}
-q \log\left(\frac{\xi_1\epsilon_n}{3qb_2}\right)&=q \log\left(\frac{3qb_2}{\xi_1\epsilon_n}\right)\\
&\lesssim q \log\left(\frac{n^{1/2}\max\{n,Q\}q }{\sqrt{\max\{s_0^\Omega,s_0^B,p,q\}\log(q)}}\right)\\
&\le q \log\left(n^{1/2}\max\{n,Q\}q \right)\\
&\lesssim q\log(q)\\
&\lesssim n\epsilon_n^2.
\end{align*}
Combining all the results we conclude that $-\log(\Pi(\mathcal{A}_1\cap \{\Omega\succ \tau I\}))\lesssim n\epsilon_n^2$ thus the prior mass $\Pi(\mathcal{A}_1\cap \{\Omega\succ \tau I\})$ is lower bounded as stated in the lemma. 

To bound $\Pi(\mathcal{A}_2|\mathcal{A}_1)$ we used a very similar strategy as the one on $\Omega$. We can also show that mass on L1 norm ball serves as a lower bound similar to that of $\Omega$. Using the definition of KL divergence and variance, the event $\mathcal{A}_2$ can be written as
\begin{align*}
    \mathcal{A}_2=\left\{(B,\Omega): \sum_{i=1}^n||\Omega^{1/2}(B-B_0)^{\top}X_i^{\top}||_2^2\le n\epsilon_n^2, \sum_{i=1}^n||\Omega_0^{-1/2}\Omega(B-B_0)^{\top}X_i^{\top}||_2^2\le n\epsilon_n^2/2\right\}
\end{align*}

Again using the argument from \cite{Ning2020}'s Lemma 5.1. 
Both $n^{-1}\sum_{i=1}^n||\Omega^{1/2}(B-B_0)^{\top}X_i^{\top}||_2^2$ and $n^{-1}\sum_{i=1}^n||\Omega_0^{-1/2}\Omega(B-B_0)^{\top}X_i^{\top}||_2^2$ are bounded by a constant multiplier of 
\begin{align*}
n^{-1}\sum_{i=1}^n||(B-B_0)^{\top}X_i^{\top}||_2^2&=n^{-1}||X(B-B_0)||_F^2.
\end{align*}
We used the facts that $||AB||_F\le \min(||A||_2||B||_F, ||A||_F||B||_2)$ and that $\Omega$ has bounded spectrum.
Since the columns of $X$ have norm of $\sqrt{n}$, we observe that
\begin{align*}
||X\Delta_B||_F\le \sqrt{n}\sum_{j=1}^p||\Delta_{B,j,.}||_F\le \sqrt{n}\sum_{j=1}^p\sum_{k=1}^q|\beta_{j,k}-\beta_{0,j,k}|.
\end{align*}
Thus, to lower bound $\Pi(\mathcal{A}_2|\mathcal{A}_1)$, it suffices to bound $\Pi(\sum |\beta_{j,k}-\beta_{0,j,k}|\le c_1\epsilon_n)$ for some fixed constant $c_1$. 


We separate the sum based on whether the true value is 0, similar to our treatment of $\Omega$:
\begin{align*}
\sum_{jk} |\beta_{j,k}-\beta_{0,j,k}|&=\sum_{(j,k)\in S_0^B}|\beta_{j,k}-\beta_{0,j,k}|+\sum_{(j,k)\in (S_0^B)^c}|\beta_{j,k}|
\end{align*}


Arguing like we did for $\Omega$, we consider the event whose intersection is a subset of $\mathcal{A}_2$
\begin{align*}
\mathcal{B}_4&=\{ \sum_{(j,k)\in S_0^B}|\beta_{j,k}-\beta_{0,j,k}|\le \frac{c_1\epsilon_n}{2}  \}\\
\mathcal{B}_5&=\{ \sum_{(j,k)\in (S_0^B)^c}|\beta_{j,k}-\beta_{0,j,k}|\le \frac{c_1\epsilon_n}{2}  \}\\
\end{align*}
We note $\mathcal{B}_4\cap \mathcal{B}_5\subset\mathcal{A}_2.$
Since the prior for $B$ is separable and independent of $\Omega,$ we have
\begin{align*}
\Pi(\mathcal{A}_2|\mathcal{A}_1)\ge \Pi(\mathcal{B}_4|\mathcal{A}_1)\Pi(\mathcal{B}_5|\mathcal{A}_1)=\Pi(\mathcal{B}_4)\Pi(\mathcal{B}_5).
\end{align*}

We bound each term similarly to $\Omega$. 
To bound $\mathcal{B}_4,$ we use the slab component of $B$'s prior
\begin{align*}
\Pi(\mathcal{B}_4)&=\int_{\mathcal{B}_4}\prod_{(j,k)\in S_0^B}\pi(\beta_{j,k}|\theta)d\mu\\
&\ge \prod_{(j,k)\in S_0^B}\int_{|\beta_{j,k}-\beta_{0,j,k}|\le \frac{c_1\epsilon_n}{2s_0^B}}\pi(\beta_{j,k}|\theta)d\beta_{j,k}\\
&\ge \theta^{s_0^B}\prod_{(j,k)\in S_0^B}\int_{|\beta_{j,k}-\beta_{0,j,k}|\le \frac{c_1\epsilon_n}{2s_0^B}}\frac{\lambda_1}{2}\exp(-\lambda_1|\beta_{j,k}|)d\beta_{j,k}\\
&\ge \theta^{s_0^B}\exp(-\lambda_1\sum_{(j,k)\in S_0^B}|\beta_{0,j,k}|)\prod_{(j,k)\in S_0^B}\int_{|\beta_{j,k}-\beta_{0,j,k}|\le \frac{c_1\epsilon_n}{2s_0^B}} \frac{\lambda_1}{2}\exp(-\lambda_1|\beta_{j,k}-\beta_{0,j,k}|)d\beta_{j,k}\\
&=\theta^{s_0^B}\exp(-\lambda_1\sum_{(j,k)\in S_0^B}|\beta_{0,j,k}|)\prod_{(j,k)\in S_0^B}\int_{|\Delta|\le \frac{c_1\epsilon_n}{2s_0^B}} \frac{\lambda_1}{2}\exp(-\lambda_1|\Delta|)d\Delta\\
&\ge \theta^{s_0^B}\exp(-\lambda_1||B_{0,S_0^B}||_1)\left[e^{-\frac{c_1\lambda_1\epsilon_n}{2s_0^B}}\frac{c_1\epsilon_n}{2s_0^B}\right]^{s_0^B}
\end{align*}
In the last line, we used Markov's inequality.
Arguing like before, we can use the spike component of $B$'s prior to control $\P(\mathcal{B}_{5})$:
\begin{align*}
\Pi(\mathcal{B}_5)&\ge (1-\theta)^{pq-s_0^B}\left[1-\frac{2(pq-s_0^B)c_1}{\epsilon_n\lambda_0}\right]^{pq-s_0^B}\\
&\gtrsim (1-\theta)^{pq-s_0^B}
\end{align*}

Combining the bounds for $\mathcal{B}_4$ and $\mathcal{B}_5,$ we obtain
\begin{align*}
-\log(\Pi(\mathcal{A}_2|\mathcal{A}_1))&\le -\log(\Pi(\mathcal{B}_4))-\log(\Pi(\mathcal{B}_5))\\
&=-\log(\theta^{s_0^B}(1-\theta)^{pq-s_0^B})+\lambda_1||B_{0,S_0^B}||_1+\frac{\lambda_1c_1\epsilon_n}{2}-s_B^0\log\left(\frac{c_1\epsilon_n}{2s_0^B}\right).
\end{align*}

By assumption on the L$_\infty$ norm of $B_0$, we have the entry of $B_0$ is bounded thus the second term $\lambda_1||B_{0,S_0^B}||_1=O(s_0^B)\lesssim n\epsilon_n^2$. The last two terms are $O(\epsilon_n)\lesssim n\epsilon_n^2$.

Recall that we tuned $\frac{1-\theta}{\theta}\sim (pq)^{2+b}$ for some $b>0.$
That is, there are constants $M_{3}$ and $M_{4}$ such that $M_3(pq)^{2+b}\le \frac{1-\theta}{\theta} \le M_4(pq)^{2+b}\le \frac{1-\theta}{\theta}$. 
The resulting bounds on $\theta$ imply that
%These bounds imply that
%$$
%1/(1+M_4(pq)^{2+b})\le \theta \le 1/(1+M_3(pq)^{2+b}),
%$$, which in turn yields
\begin{align*}
    \theta^{s_0^B}(1-\theta)^{pq-s_0^B}&\ge(1+M_4(pq)^{2+b})^{-s_0^B}(1-\theta)^{pq-s_0^B}\\
    &\ge(1+M_4(pq)^{2+b})^{-s_0^B}\left(1-1/(1+M_3(pq)^{2+b})\right)^{pq-s_0^B}\\
    &\gtrsim (1+M_4(pq)^{2+b})^{-s_0^B}
  \end{align*}
    
The last line follows because $(pq)^{2+\beta}$ grows faster than $pq-s_0^B.$ 
Thus $\left(1-1/(1+M_3(pq)^{2+b})\right)^{pq-s_0^B}$ can be bounded from below with some constant not depending on $n$. 
Consequently,
    \begin{align*}
    -\log\left(\theta^{s_0^B}(1-\theta)^{pq-s_0^B}\right)\lesssim s_0^B\log(1+M_4(pq)^{2+b})\lesssim s_0^B\log(pq)\lesssim s_0^B\max\{\log(q),\log(p)\}
    \end{align*}

    To bound the last term we write out $\epsilon_n$ 
\begin{align*}
    -s_B^0\log\left(\frac{c_1\epsilon_n}{2s_0^B}\right)&=s_B^0\log\left(\frac{2s_0^B}{c_1\epsilon_n}\right)\\
    &\lesssim s_0^B\log\left(\frac{\sqrt{n}s_0^B}{\sqrt{\max\{q,s_0^B,s_0^\Omega\}\log(\max\{p,q\})}}\right)\\
    &\le s_0^B\log(\sqrt{n s_0^B})\\
    &\lesssim s_0^B\log(pq)\\
    &\lesssim n\epsilon_n^2
\end{align*}
The third line used the fact when $n$ large $\log(\max\{p,q\})>1$ and the last two lines follow from our assumption that $\log(n)\lesssim \log(q)$ and $s_0^B< pq$. 

Combining all these results, the prior mass $\Pi(\mathcal{A}_2|\mathcal{A}_1)$ can be lower bounded as stated. 


\subsection{Proof of Lemma 2}

The main idea is to check the posterior probability directly. 
Let $\mathcal{B}^B_n=\{B:|\nu_{\beta}(B)|<r^B_n\}$ for some $r_n^B=C_3'\max\{q,s_0^B,s_0^\Omega\}$ with $C_3'>C_1$ in the KL condition. 
For $\Omega$, let $\mathcal{B}^\Omega_n=\{\Omega\succ \tau I:|\nu_{\omega}(\Omega)|<r^\Omega_n\}$ for $r_n^\Omega=C_3'\max\{q,s_0^B,s_0^\Omega\}$ with some $C_3'>C_1$ in the KL condition. 
We aim to show that $\E_0\Pi(\Omega\in(\mathcal{B}^\Omega_n)^c|Y_1,\dots,Y_n )\to 0$ and $\E_0\Pi(B\in(\mathcal{B}^B_n)^c|Y_1,\dots,Y_n )\to 0$.

The marginal posterior can be expressed using log-likelihood $\ell_n$:
\begin{equation}
    \label{eqn:posterior_B_m}
    \begin{aligned}
        \Pi(B\in \mathcal{B}_n^B|Y_1,\dots,Y_n)&=\frac{\iint_{\mathcal{B}_n^B}\exp(\ell_n(B,\Omega)-\ell_n(B_0,\Omega_0))d\Pi(B)d\Pi(\Omega)}{\iint\exp(\ell_n(B,\Omega)-\ell_n(B_0,\Omega_0))d\Pi(B)d\Pi(\Omega)}\\
        \Pi(\Omega\in \mathcal{B}_n^\Omega|Y_1,\dots,Y_n)&=\frac{\iint_{\mathcal{B}_n^\Omega}\exp(\ell_n(B,\Omega)-\ell_n(B_0,\Omega_0))d\Pi(B)d\Pi(\Omega)}{\iint\exp(\ell_n(B,\Omega)-\ell_n(B_0,\Omega_0))d\Pi(B)d\Pi(\Omega)}
    \end{aligned}
\end{equation}


By using the result of KL condition (Lemma \ref{lemma:KL_m}), we can, with high probability, bound the denominator from below by $e^{-C_1n\epsilon_n^2}.$
Consequently, focus now on upper bounded the numerators in these expressions, starting with $B.$
\begin{align*}
    \E_0\left(\iint_{(\mathcal{B}_n^{B})^c}f/f_0d\Pi(B)d\Pi(\Omega)\right)
    \le \int_{(\mathcal{B}_n^{B})^c}d\Pi(B)=\Pi(|\nu_{\beta}(B)|\ge r_n^B).
\end{align*}

Notice that when $|\beta_{j,k}|>\delta_\beta,$ we have $\pi(\beta_{j,k})<2\theta\frac{\lambda_1}{2}\exp(-\lambda_1|\beta_{j,k}|).$
Therefore, we can bound the above display as follows
\begin{align*}
    \Pi(|\nu_{\beta}(B)|\ge r_n^B)&\le \sum_{|S|>r_n^B}(2\theta)^{|S|}\prod_{(j,k)\in S}\int_{|\beta_{j,k}|>\delta_\beta} \frac{\lambda_1}{2}\exp(-\lambda_1|\beta_{j,k}|) d\beta_{j,k} \prod_{(j,k)\notin S} \int_{|\beta_{j,k}|<\delta_\beta}\pi(\beta_{j,k})d\beta_{j,k}\\
    &\le \sum_{|S|>r_n^B}(2\theta)^{|S|}\\
\end{align*}
Using the assumption on $\theta$, and the fact $\binom{pq}{k}\le (epq/k)^k$ (similar to \citet{Bai2020_groupSSL}'s Equation D.32), we can further upper bound the probability:
\begin{align*}
    \Pi(|\nu_{\beta}(B)|\ge r_n^B)&\le \sum_{|S|>r_n^B}(2\theta)^{|S|}
    \le \sum_{|S|>r_n^B}(\frac{2}{1+M_4 (pq)^{2+b}})^{|S|}\\
    &\le \sum_{k=\left\lfloor r_n^B\right\rfloor +1}^{pq} \binom{pq}{k}\left(\frac{2}{M_4(pq)^2}\right)^k
    \le \sum_{k=\left\lfloor r_n^B\right\rfloor +1}^{pq} \left(\frac{2e}{M_4kpq}\right)^k\\
    &<\sum_{k=\left\lfloor r_n^B\right\rfloor +1}^{pq} \left(\frac{2e}{M_4(\left\lfloor r_n^B\right\rfloor +1)pq}\right)^k\\
    &\lesssim (pq)^{-(\left\lfloor r_n^B\right\rfloor +1)}\\
    %&=\exp(-(\left\lfloor r_n^B\right\rfloor +1)\log(pq))\\
    &\le \exp(-(\left\lfloor r_n^B\right\rfloor)\log(pq)).
\end{align*}
Taking $r_n^B=C_3'\max\{q,s_0^B,s_0^\Omega\}$ for some $C_3'>C_1$, we have:
\begin{align*}
    \Pi(|\nu_{\beta}(B)|\ge r_n^B)&\le \exp(-C_3'\max\{q,s_0^B,s_0^\Omega\}\log(pq)).
\end{align*}
Therefore
\begin{align*}
    \E_0\Pi((\mathcal{B}_n^B)^c|Y_1,\dots,Y_n)\le \E_0\Pi((\mathcal{B}_n^B)^c|Y_1,\dots,Y_n)I_{E_n}+\P_0(E_n^c),
\end{align*}
where $E_n$ is the event in KL condition. 
On the event $E_n$, the KL condition ensures that the denominator in Equation~\eqref{eqn:posterior_B_m} is lower bounded by $\exp(-C_1n\epsilon_n^2)$ and is upper bounded by $\exp(-C_3'\max\{q,s_0^B,s_0^\Omega\}\log(pq)).$
Further since $\P_0(E_n^c)\to 0$, we conclude that
\begin{align*}
    \E_0\Pi((\mathcal{B}_n^B)^c|Y_1,\dots,Y_n)&\le \exp(C_1n\epsilon_n^2-C_3'\max\{q,s_0^B,s_0^\Omega\}\log(pq))+o(1)\to 0
\end{align*}
The workflow for $\Omega$ is very similar, except we need to use the upper bound of the graphical prior in Equation~\eqref{eqn:graphical_prior_bound} to properly bound the prior mass of the set with overestimated dimensionality of $\Omega$. 

We upper bound the numerator:
\begin{align*}
    \E_0\left(\iint_{(\mathcal{B}_n^{\Omega})^c}f/f_0d\Pi(B)d\Pi(\Omega)\right)&\le \int_{(\mathcal{B}_n^{\Omega})^c}d\Pi(\Omega)=\Pi(|\nu_{\omega}(\Omega)|\ge r_n^\Omega)\le \exp(2\xi_1 Q-\log(R))\tilde{\Pi}(|\nu_{\omega}(\Omega)|\ge r_n^\Omega)
\end{align*}

Whenever $|\omega_{k,k'}|>\delta_\omega,$ we know $\pi(\omega_{k,k'})<2\eta\frac{\xi_1}{2}\exp(-\xi_1|\omega_{k,k'}|)$, yielding the bound 
\begin{align*}
    \tilde{\Pi}(|\nu_{\omega}(\Omega)|\ge r_n^\Omega)&\le \sum_{|S|>r_n^\Omega}(2\eta)^{|S|}\prod_{(k,k')\in S}\int_{|\omega_{k,k'}|>\delta_\omega} \frac{\xi_1}{2}\exp(-\xi_1|\omega_{k,k'}|) d\omega_{k,k'} \prod_{(k,k')\notin S} \int_{|\omega_{k,k'}|<\delta_\omega}\pi(\omega_{k,k'})d\omega_{k,k'}\\
    &\le \sum_{|S|>r_n^\Omega}(2\eta)^{|S|}
\end{align*}

By using the assumption on $\eta$, and the fact $\binom{Q}{k}\le (eQ/k)^k$, we further bound
\begin{align*}
    \tilde{\Pi}(|\nu_{\omega}(\Omega)|\ge r_n^\Omega)&\le \sum_{|S|>r_n^\Omega}(2\eta)^{|S|}
    \le \sum_{|S|>r_n^\Omega}(\frac{2}{1+K_4 Q^{2+b}})^{|S|}\\
    &\le \sum_{k=\left\lfloor r_n^\Omega\right\rfloor +1}^{Q} \binom{Q}{k}\left(\frac{2}{K_4Q^2}\right)^k
    \le \sum_{k=\left\lfloor r_n^\Omega\right\rfloor +1}^{Q} \left(\frac{2e}{K_4kQ}\right)^k\\
    &<\sum_{k=\left\lfloor r_n^\Omega\right\rfloor +1}^{Q} \left(\frac{2e}{K_4(\left\lfloor r_n^\Omega\right\rfloor +1)Q}\right)^k\\
    &\lesssim Q^{-(\left\lfloor r_n^\Omega\right\rfloor +1)}\\
    %&=\exp(-(\left\lfloor r_n^\Omega\right\rfloor +1)\log(Q))\\
    &\le \exp(-(\left\lfloor r_n^\Omega\right\rfloor)\log(Q)).
\end{align*}

Taking $r_n^\Omega=C_3'\max\{q,s_0^B,s_0^\Omega\}$ with $C_3'>C_1$, we have:
\begin{align*}
    \tilde{\Pi}(|\nu_{\omega}(\Omega)|\ge r_n^\Omega)&\le \exp(-C_3'\max\{q,s_0^B,s_0^\Omega\}\log(Q))\le \exp(-C_3'n\epsilon_n^2).
\end{align*}

Using the assumption that $\xi_1 \asymp 1/\max\{Q,n\},$ for some $R'$ not depending on $n$ we conclude that
\begin{align*}
    \Pi(|\nu_{\omega}(\Omega)|\ge r_n^\Omega)\le \exp(-C_3n\epsilon_n^2+2\xi_1 Q-\log(R))\le \exp(-C_3'n\epsilon_n^2+\log(R')).
\end{align*}

Therefore,
\begin{align*}
    \E_0\Pi((\mathcal{B}_n^\Omega)^c|Y_1,\dots,Y_n)\le \E_0\Pi((\mathcal{B}_n^\Omega)^c|Y_1,\dots,Y_n)I_{E_n}+P_0(E_n^c),
\end{align*}
where $E_n$ is the event in KL condition. 
On $E_n$, the KL condition ensures that the denominator in Equation~\eqref{eqn:posterior_B_m} is lower bounded by $\exp(-C_1n\epsilon_n^2)$ and is upper bounded by $\exp(-C_3'n\epsilon_n^2+\log(R')).$ 
Further since $P_0(E_n^c)\to 0$, we obtain the following lower bound
\begin{align}
    \E_0\Pi((\mathcal{B}_n^\Omega)^c|Y_1,\dots,Y_n)&\le \exp(C_1n\epsilon_n^2-C_3'n\epsilon_n^2+\log(R'))+o(1)\to 0
    \label{eq:Omega_dimension}
\end{align}


\subsection{Proof of Lemma 3 and 4}


%We will need Lemma~\ref{lemma:packing_number_lp}, by \citet{shen2022cgSSL}, provides a bound for these covering numbers. %and we restate it here.
We will need Lemma 5, which provides a bound for these covering numbers. %and we restate it here.



\subsubsection{Lemma 3}

We show the first part of Lemma 3 that 
\begin{equation}
    \mathcal{F}_n=\left\{B\in \mathcal{B}^B_n,\Omega\in \mathcal{B}^\Omega_n:||B||_1\le 2C_3p, ||\Omega||_1 \le 8C_3q \right\}
\end{equation}
for some large $C_3>C_1+2+\log(3)$ where $C_1$ is the constant in KL condition. 
We have
\begin{align*}
    \Pi(\mathcal{F}_n^c)&\le \Pi(||B||_1> 2C_3p)+\Pi((||\Omega||_1 > 8C_3q)\cap \{\Omega\succ \tau I\}).
\end{align*}

We upper bound each term. 
Using the bound in Equation~\eqref{eqn:graphical_prior_bound}, we have
\begin{align*}
    \Pi((||\Omega||_1 > 8C_3q)\cap \{\Omega\succ \tau I\})\le \exp(2\xi_1 Q-\log(R))\tilde{\Pi}(||\Omega||_1 > 8C_3q).
\end{align*}

Since $||\Omega||_1=2\sum_{k>k'}|\omega_{k,k'}|+\sum_{k}|\omega_{k,k}|$, at least one of these two sums exceeds $8C_3q/2$. Thus, we can form an upper bound on the L1 norm probability
\begin{align*}
    \tilde{\Pi}\left(||\Omega||_1 > 8C_3q\right)\le \tilde{\Pi}\left(\sum_{k>k'}|\omega_{k,k'}|>\frac{8C_3q}{4}\right)+\tilde{\Pi}\left(\sum_{k}|\omega_{k,k}|>\frac{8C_3q}{2}\right).
\end{align*}

Under $\tilde{\Pi}$, the slab distribution provides an an upper bound, where $\sum_{k>k'}|\omega_{k,k'}|$ is Gamma distributed with shape parameter $Q$ and rate parameter $\xi_1$. 
By using an appropriate tail estimation of Gamma distribution (\citet{boucheron2013concentration}, pp.29), and the fact $1+x-\sqrt{1+2x}\ge (x-1)/2,$ we compute
\begin{align*}
    \exp(2\xi_1 Q-\log(R))\tilde{\Pi}(\sum_{k>k'}|\omega_{k,k'}| > 8C_3q/4)&\le \exp\left[-Q\left(1-\sqrt{1+2\frac{8C_3q}{4Q\xi_1}}+\frac{8C_3q}{4Q\xi_1}\right)+2Q-\log(R)\right]\\
    &\le \exp\left[-\frac{8C_3q}{8\xi_1}+\left(\frac{5}{2}Q-\log(R)\right)\right].
\end{align*}

Using the fact $\xi_1\asymp 1/\max\{n,Q\}$, we have as $n$ sufficiently large, $ n\epsilon_n^2\ge q\log(q)$ thus $qn\epsilon_n^2\ge Q\log(q)$ and $Q=o(qn\epsilon_n^2)$, 
\begin{align*}
    \frac{8C_3q}{8\xi_1}-\left(\frac{5}{2}Q-\log(R)\right)&\asymp C_3(\max\{n,Q\}q)-\left(\frac{5}{2}Q-\log(R)\right)\\
    &\ge C_3(qn\epsilon_n^2)-\left(\frac{5}{2}Q-\log(R)\right)\\
    &=C_3(qn\epsilon_n^2)-o(qn\epsilon_n^2)\\
    &\ge C_3n\epsilon_n^2.
\end{align*}

The first order term of $Q$ on the left hand side can be ignored when $n$ large as the left hand side is dominated by the $Q\log(q)$ term. We have also used the assumption that $\epsilon_n\to 0$. 
Thus we have,
\begin{align*}
    \exp(2 \xi_1 Q-\log(R))\tilde{\Pi}((\sum_{k>k'}|\omega_{k,k'}| > 8C_3q/4))\le \exp(-C_3n\epsilon_n^2).
\end{align*}

For the diagonal, the sum is gamma distributed with shape $q$ and rate $\xi_1$, yielding a similar bound:
\begin{align*}
    \exp(2 \xi_1 Q-\log(R))\tilde{\Pi}(\sum_{k}|\omega_{k,k}| > 8C_3q/2)&\le \exp(2 Q-\log(R))\exp\left[-q\left(1-\sqrt{1+2\frac{8C_3q}{2q\xi_1}}+\frac{8C_3q}{2q\xi_1}\right)\right]\\
    &\le \exp\left[-\frac{8C_3q}{4\xi_1}+Q\left(2+\frac{q}{2Q}\right)-\log(R)\right].
\end{align*}

By using the same argument as before and the fact that $\xi_1 \asymp 1/\max\{Q,n\},$ we have
\begin{align*}
\frac{8C_3q}{4\xi_1}-Q\left(2+\frac{q}{2Q}\right)+\log(R)&\asymp 2C_3(\max\{Q,n\}q))-Q\left(2+\frac{q}{2Q}\right)+\log(R)\\
&\ge  C_3qn\epsilon_n^2-o(qn\epsilon_n^2)\\
&\ge C_3n\epsilon_n^2.
\end{align*}

The first order term of $Q$ on the left hand side can be ignored when $n$ large as the left hand side is dominated by the $Q\log(q)$ term and $q/Q\to 0$. 
By combining the above results, we have 
\begin{equation}
\label{eqn:sieve_Omega_bound_mssl}
\begin{aligned}
	\Pi((||\Omega||_1 > 8C_3q)\cap \{\Omega\succ \tau I\})\le& \exp(2 Q-\log(R))\tilde{\Pi}(||\Omega||_1 > 8C_3q)\\
	\le& \exp(2 Q-\log(R))\tilde{\Pi}(\sum_{k>k'}|\omega_{k,k'}|>\frac{8C_3q}{4})\\
    &+\exp(2 Q-\log(R))\tilde{\Pi}(\sum_{k}|\omega_{k,k}|>\frac{8C_3q}{2})\\
	\le& 2\exp(-C_3n\epsilon_n^2).
\end{aligned}
\end{equation}
The probability $||B||_1>2C_3p$ can be bound by tail probability of Gamma distribution with shape parameter $pq$ and rate parameter $\lambda_1$:
\begin{align*}
	\Pi(||B||_1> 2C_3p)&\le \exp\left[-pq\left(1-\sqrt{1+2\frac{2C_3p}{pq\lambda_1}}+\frac{2C_3p}{pq\lambda_1}\right)\right]\\
	&\le  \exp\left[-pq\left(\frac{2C_3p}{2pq\lambda_1}-\frac{1}{2}\right)\right]\\
	&\le \exp\left(-\frac{2C_3p}{2\lambda_1}+\frac{pq}{2}\right).
\end{align*}
Using the same argument, we have, $pn\ge pn\epsilon_n^2\ge pq\log(q)$ so $pq=o(pn\epsilon_n^2)$ for large $n$, and
\begin{align*}
	\exp\left(-\frac{2C_3p}{2\lambda_1}+\frac{pq}{2}\right)\le \exp\left(-C_3pn\epsilon_n^2+o(pn\epsilon_n^2)\right)\le \exp(-C_3n\epsilon_n^2).
\end{align*}

Combining these two inequalities, we have
\begin{equation}
\label{eqn:sieve_B_bound_mssl}
\begin{aligned}
	\Pi(||B||_1> 2C_3p)&\le\exp\left(-\frac{2C_3p}{2\lambda_1}+\frac{pq}{2}\right) \le\exp(-C_3n\epsilon_n^2)
\end{aligned}
\end{equation}

By combining the result from Equations~\eqref{eqn:sieve_Omega_bound_mssl} and~\eqref{eqn:sieve_B_bound_mssl}, we have
\begin{align*}
	\Pi(\mathcal{F}_n^c)\le 3\exp(-C_3n\epsilon_n^2)=\exp(-C_3n\epsilon_n^2+\log(3)).
\end{align*}
With our choice of $C_3$, the above probability is asymptotically bounded from above by $\exp(-C_2n\epsilon_n^2)$ for some $C_2\ge C_1+2$. 

\subsubsection{Lemma 5}

Here we give the proof of lemma 5. 

Instead of directly constructing the $\varphi_n$ whose alternative is the whole sieve, we start by constructing a sequence of tests whose alternative correspond tp representative points. 
We show that these tests have bounded Type II error in the neighborhood of the representative points.
We can then construct a test against the entire sieve by taking the supremum of the tests constructed against representative points. 
We finally apply the general theory by bounding the number of neighborhoods around representative points needed to cover the entire sieve. 

For a representative point $f_1$, we consider the Neyman-Pearson test against a single point alternative $H_0: f=f_0, H_1: f=f_1$, $\phi_n=I\{ f_1/f_0\ge 1 \}$. 
If the average half-order R\'enyi divergence $-n^{-1}\log(\int\sqrt{f_0f_1}d\mu)\ge \epsilon^2$,  we will have:
\begin{align*}
    \mathbb{E}_{f_0}(\phi_n)&\le\int_{f_1>f_0}\sqrt{f_1/f_0} f_0 d\mu\le \int \sqrt{f_1f_0}d\mu\le e^{-n\epsilon^2}\\
    \mathbb{E}_{f_1}(1-\phi_n)&\le\int_{f_0>f_1}\sqrt{f_0/f_1} f_1 d\mu\le \int \sqrt{f_0f_1}d\mu\le e^{-n\epsilon^2}.
\end{align*}
By Cauchy-Schwarz, for any alternative $f$ we can control the type-II error rate:
\begin{align*}
    \E_f(1-\phi_n)\le \{\E_{f_1}(1-\phi_n)\}^{1/2}\{\E_{f_1}(f/f_1)^2\}^{1/2}.
\end{align*}
So long as the second factor grows at most like $e^{cn\epsilon^2}$ for some properly chosen small $c$, the full expression can be controlled.  
Thus we can consider the neighborhood around the representative point small enough so that the second factor can be actually bounded.

Consider every density with parameters satisfying
\begin{equation}
    \label{eqn:test_sets_mssl}
    \begin{aligned}
    &|||\Omega|||_2\le ||\Omega||_1\le 8C_3q,\\
    &||B_1-B||_2\le ||B_1-B||_1\le \frac{1}{\sqrt{2C_3npq}},\\
    &|||\Omega_1-\Omega|||_2\le ||\Omega_1-\Omega||_1\le \frac{1}{8C_3nq^{3/2}}.
\end{aligned}
\end{equation}

We show that $\E_{f_1}(f/f_1)^2$ is bounded on the above set when parameters are from the sieve $\mathcal{F}_n$. 
Denote $\Sigma_1=\Omega_1^{-1}$, $\Sigma=\Omega^{-1}$ as well as $\Sigma_1^\star=\Omega^{1/2}\Sigma_1\Omega^{1/2}$, and $\Delta_B=B-B_1$ while $\Delta_\Omega=\Omega-\Omega_1$. 
\begin{align}
    \begin{split}
    \label{eqn:test_f_over_f1_mssl}
        \E_{f_1}(f/f_1)^2=&|\Sigma_1^\star|^{n/2}|2I-\Sigma_1^{\star-1}|^{-n/2}\\
        &\times \exp\left(\sum_{i=1}^nX_i(B-B_1)\Omega^{1/2}(2\Sigma_1^\star-I)^{-1}\Omega^{1/2}(B-B_1)^{\top}X_i^{\top}\right).
    \end{split}
\end{align}
For the first factor, 
%we use the same argument as in \citet[Equation 5.9]{Ning2020}. 
since $\Omega\in\mathcal{F}_n$, we have $|||\Omega^{-1}|||_2\le 1/\tau.$
The fact that $|||\Omega_1-\Omega|||_2\le \delta_n'= 1/8C_3nq^{3/2}$ implies that
\begin{align*}
    |||\Sigma_1^\star-I|||_2\le |||\Omega^{-1}|||_2|||\Omega_1-\Omega|||_2\le \delta_n'/\tau.
\end{align*}
We can therefore bound the spectrum of $\Sigma_1^\star$, i.e. $1-\delta_n'/\tau\le \eig_1(\Sigma_1^\star)\le \eig_q(\Sigma_1^\star)\le  1+\delta_n'/\tau $.

Thus
\begin{align*}
    \left(\frac{|\Sigma_1^\star|}{|2I-\Sigma_1^{\star-1}|}\right)^{n/2}&=\exp\left(\frac{n}{2}\sum_{i=1}^q\log(\eig_i(\Sigma_1^\star))-\frac{n}{2}\sum_{i=1}^q \log\left(2-\frac{1}{\eig_i(\Sigma_1^\star)}\right)\right)\\
    &\le \exp\left(\frac{nq}{2}\log(1+\delta_n'/\tau)-\frac{nq}{2}\log\left(1-\frac{\delta_n'/\tau}{1-\delta_n'/\tau}\right)\right)\\
    &\le \exp\left(\frac{nq^2}{2}\delta_n'+\frac{nq}{2}\left(\frac{\delta_n'/\tau}{1-2\delta_n'/\tau}\right)\right)\\
    &\le \exp(nq\delta_n'/\tau)\\
    &\le e
\end{align*}
The third inequality follows from the fact $1-x^{-1}\le \log(x)\le x-1$.

We can bound the log of the second factor by
\begin{align*}
    |||\Omega|||_2|||(2\Sigma_1^\star-I)^{-1}|||_2\sum_{i=1}^n||X_i\Delta_B||_2^2\le 16C_3q \sum_{i=1}^n||X_i\Delta_B||_2^2\le 16C_3npq ||\Delta_B||_2^2\le 8
\end{align*}
The desired test $\varphi_n$ in Lemma \ref{lemma:test-condition} can be obtained as the maximum of all tests $\phi_n$ described above -- that is, the maximum over all sets defined in Equation~\eqref{eqn:test_sets_mssl} that covers the sieve $\mathcal{F}_n$.


To finish the proof, we use a covering arguments to show that $\phi_n$'s we take maximum over is not too big. Formally we show that number of sets described in Equation~\eqref{eqn:test_sets_mssl} needed to cover sieve $\mathcal{F}_n$, denoted by $N_*$, can be bounded by $\exp(Cn\epsilon_n^2)$ for some suitable constant $C$. 

We can bound the logarithm of the covering number $\log(N_*)$:
\begin{align*}
    \log(N_*)\le & \log\left[N\left(\frac{1}{\sqrt{2C_3npq}},\{B\in \mathcal{B}^B_n:||B||_1\le2C_3p\},||\cdot||_1\right)\right]\\
    &+\log\left[N\left(\frac{1}{8C_3nq^{3/2}},\{\Omega \in \mathcal{B}^\Omega_n,||\Omega||_1\le 8C_3q\},||\cdot||_1\right)\right]
\end{align*}
The two terms above can be treated in a similar fashions. 
Denote $\max\{q,s_0^B,s_0^\Omega\}=s^\star$. 
Since there are multiple ways to allocate the effective 0's, we pick up a binomial coefficient below:
\begin{equation}   
\begin{aligned}
    &N\left(\frac{1}{8C_3n q^{3/2}},\{\Omega \in \mathcal{B}^\Omega_n,||\Omega||_1\le 8C_3q\},||\cdot||_1\right)\\
    \le & \binom{Q}{C_3's^\star} N\left(\frac{1}{8C_3nq^{3/2}},\{V\in \mathbb{R}^{Q+q}:|v_i|<\delta_\omega\text { for $1\le i\le Q+q-C_3's^\star$},||V||_1\le 8C_3q\},||\cdot||_1\right) \label{eq:covering_Omega} \\
    &N\left(\frac{1}{\sqrt{2C_3npq}},\{B\in \mathcal{B}^B_n:||B||_1\le2C_3p\},||\cdot||_1\right)\\
    \le & \binom{pq}{C_3' s^\star}  N\left(\frac{1}{\sqrt{2C_3npq}},\{V\in \mathbb{R}^{pq}:|v_i|<\delta_\beta\text { for $1\le i\le pq-C_3's^\star$},||V||_1\le 2C_3p\},||\cdot||_1\right).
\end{aligned}
\end{equation}

Note that $\Omega$ has $Q+q<2Q$  free parameters. 
We have first
\begin{align*}
    \log \binom{Q}{C_3's^\star}&\lesssim s^\star \log(Q)\lesssim n\epsilon_n^2 \\
    \log \binom{pq}{C_3's^\star}&\lesssim s^\star \log(pq)\lesssim n\epsilon_n^2. 
\end{align*}

Observe that for $V' \in \R^{C_{3}'s^{\star}}$, we have
$$||V||_1\cap \{|v_i|<\delta_\omega \text{ for } 1\le i\le Q+q-C_3's^\star\}\subset \{||V'||\le 8C_3q\}\times[-\delta_\omega,\delta_\Omega]^{Q+q-C_3's^\star}.
$$
Thus,
\begin{align*}
    &N\left(\frac{1}{8C_3nq^{3/2}},\{V:|v_i|<\delta_\omega\text { for $1\le i\le Q+q-C_3's^\star$},||V||_1\le 8C_3q\},||\cdot||_1\right)\\
    \le & N\left(\frac{1}{8C_3nq^{3/2}},\{V\in \mathbb{R}^{C_3's^\star}:||V'||_1\le 8C_3q\times [-\delta_\omega,\delta_\omega]^{Q+q-C_3's^\star}\},||\cdot||_1\right)\\
\end{align*}

Because we are covering the sieve with $L_{1}$-norm balls, we will verify the condition of Lemma 5 with $p = 1$ and $T = 2.$
The choice $T=2$ is arbitrary but makes the calculation easy. 
By our assumption on $\xi_0$, we have
\begin{align*}
    (Q+q-C_3's^\star)\delta_\omega&\le 2Q\delta_\omega = 2Q\frac{1}{\xi_0-\xi_1}\log\left[\frac{1-\eta}{\eta}\frac{\xi_0}{\xi_1}\right]\lesssim  \frac{Q\log(\max\{q,n\})}{\max\{Q,n\}^{4+b/2+b/2}}\\
    &\le \frac{1}{\max\{Q,n\}^{3+b/2}}
\end{align*}
The denominator dominates $ C_3nq^{3/2}$ thus for large enough $n$, we have $(Q+q-C_3's^\star)\delta_\omega\le \frac{1}{32C_3nq^{3/2}}$ thus by Lemma 5, we can control the covering number by the packing number:
\begin{align*}
    &
    \log N\left(\frac{1}{8C_3nq^{3/2}},\{V:|v_i|<\delta_\omega\text { for $1\le i\le Q+q-C_3's^\star$},||V||_1\le 8C_3q\},||\cdot||_1\right)\\
    \le &\log D\left(\frac{1}{16C_3nq^{3/2}},\{V'\in \mathbb{R}^{C_3's^\star},||V'||_1\le 8C_3q\},||\cdot||_1\right)\\
    \lesssim & s^\star \log(128C_3^2qnq^{3/2})\\
    %\le &2(s^\star) \log(128C_3^2qnq^{3/2})\\
    \lesssim& n\epsilon_n^2.
\end{align*}

We treat the covering number for $B$ in a similar fashion:
\begin{align*}
    &N\left(\frac{1}{\sqrt{2C_3npq}},\{V:|v_i|<\delta_\beta\text { for $1\le i\le pq-C_3's^\star$},||V||_1\le 2C_3p\},||\cdot||_1\right)\\
    \le& N\left(\frac{1}{\sqrt{2C_3npq}},\{V'\in \mathbb{R}^{C_3's^\star}:||V'||_1\le 2C_3p\times [-\delta_\beta,\delta_\beta]^{pq-C_3's^\star}\},||\cdot||_1\right)
\end{align*}

%We once again verify the condition of Lemma~\ref{lemma:packing_number_lp} with $p=1$ and $T=2$:
We once again verify the condition of Lemma 5 with $p=1$ and $T=2$:
\begin{align*}
    (pq-C_3's^\star )\delta_\beta&\le pq\delta_\beta=\frac{pq}{\lambda_0-\lambda_1}\log\left[\frac{1-\theta}{\theta}\frac{\lambda_0}{\lambda_1}\right]\lesssim \frac{pq\log(\max\{p,q,n\})}{\max\{pq,n\}^{5/2+b/2+b/2}}\\
    &\le \frac{1}{\max\{pq,n\}^{3/2+b/2}}.
\end{align*}
The denominator dominates $\sqrt{2C_3npq}$, Thus for enough large $n$, we have $(pq-C_3's^\star )\delta_\beta\le 1/4\sqrt{2C_3npq}$. Thus similar to $\Omega$, we have:
\begin{align*}
    &
    \log N\left(\frac{1}{\sqrt{2C_3npq}},\{V:|v_i|<\delta_\omega\text { for $1\le i\le pq-C_3's^\star$},||V||_1\le 2C_3p\},||\cdot||_1\right)\\
    \le &\log D\left(\frac{1}{2\sqrt{2C_3npq}},\{V'\in \mathbb{R}^{C_3's^\star},||V'||_1\le 2C_3p\},||\cdot||_1\right)\\
    \lesssim & s^\star \log(4C_3p\sqrt{2C_3npq})\\
    \lesssim& n\epsilon_n^2.
\end{align*}



